Identifying Explanation Needs of End-users: Applying and Extending the XAI Question Bank

Explanations in XAI are typically developed by AI experts and focus on algorithmic transparency and the inner workings of AI systems. Research has shown that such explanations do not meet the needs of users who do not have AI expertise. As a result, explanations are often ineffective in making system decisions interpretable and understandable. We aim to strengthen a socio-technical view of AI by following a Human-Centered Explainable Artificial Intelligence (HC-XAI) approach, which investigates the explanation needs of end-users (i.e., subject matter experts and lay users) in specific usage contexts. One of the most influential works in this area is the XAI Question Bank (XAIQB) by Liao et al. The authors propose a set of questions that end-users might ask when using an AI system, which in turn is intended to help developers and designers identify and address explanation needs. Although the XAIQB is widely referenced, there are few reports of its use in practice. In particular, it is unclear to what extent the XAIQB sufficiently captures the explanation needs of end-users and what potential problems exist in the practical application of the XAIQB. To explore these open questions, we used the XAIQB as the basis for analyzing 12 think-aloud software explorations with subject matter experts. We investigated the suitability of the XAIQB as a tool for identifying explanation needs in a specific usage context. Our analysis revealed a number of explanation needs that were missing from the question bank, but that emerged repeatedly as our study participants interacted with an AI system. We also found that some of the XAIQB questions were difficult to distinguish and required interpretation during use. Our contribution is an extension of the XAIQB with 11 new questions. In addition, we have expanded the descriptions of all new and existing questions to facilitate their use.

==> Archive_intern.tex <==
% Kritik an/Grenzen von Liao et al.
% Wichtig ist und nicht nur XAI Needs: Design Recommendations for HCI: Amershi https://doi.org/10.1145/3290605.330023 - dieses Paper zitieren Liao et al. auch, kritisieren aber, dass dort keine ``actionable guidance'' dazu angeboten wird, wie diese Möglichkeiten/Anforderungen umgesetzt werden sollen. Unser Paper zeigt (vermutlich) auf, dass XAI ohne die Betrachtung ``allgemeiner'' user needs nicht ausreicht. Daher besser: context-specific und user-specific combination of both! 

%based on expert opinions from different fields~\cite{Mohseni2021}, stakeholders needs~\cite{preece2018stakeholders, langer2021}, stakeholders knowledge and goals~\cite{suresh2021a}, and psychology~\cite{sanneman2020, Wang2019}. 
% used needs angeschaut + interview
%Other authors have used interviews to investigate user needs~\cite{Hong2020, Liao2020}. 
% sanneman2020
    % Drawing from the human factors literature
    % based on the informational needs of human users, which can be determined using the levels of situation awareness (SA) framework from the human factors literature
% Hong2020
    % conducted 22 semi-structured interviews with industry practitioners to understand how they conceive of and design for interpretability while they plan, build, and use their models
    % Based on a qualitative analysis of our results, we differentiate interpretability roles, processes, goals and strategies as they exist within organizations making heavy use of ML models
% Wang2019
    % This paper seeks to strengthen empirical application-specific investigations of XAI by exploring theoretical underpinnings of human decision making, drawing from the fields of philosophy and psychology. 
    %  theory-driven conceptual framework + An application of our framework to medical decision making to demonstrate its usefulness in designing usercentric XAI.
% suresh2021a
    % Erstellen ein Framework und evaluieren es an 58 paper
    %In this paper, we eschew prior expertise- and role-based categorizations of interpretability stakeholders in favor of a more granular framework that decouples stakeholders’ knowledge from their interpretability needs.
% preece2018stakeholders
    % Teilen Stakeholder in Gruppen auf, die unterschiedliche Needs haben
    % On a final note, the most influential of our four stake- holder communities is the users — the one that’s barely rep-resented in the literature 
    %We use the software engineering distinction between validation and verification, and the epis-temological distinctions between knowns/unknowns, to tease apart the concerns of the stakeholder communities and high-light the areas where their foci overlap or diverge
% langer2021
    % This paper discusses the main classes of stakeholders calling for explainability of artificial systems and reviews their desiderata
    % We provide a model that explicitly spells out the main concepts and relations necessary to consider and investigate when evaluating, adjusting, choosing, and developing explainability approaches that aim to satisfy stakeholders’ desiderata.



% Rike Stand 08.06.23
\section{Related Work}
% AI zu XAI need
Over the last decade, the field of Artificial Intelligence (AI) has made substantial progress and is now used in many areas. Due to increasing model complexity and the use of non-transparent black-box AI models, the field of Explainable Artificial Intelligence (XAI) has emerged to make AI decisions understandable and explainable \cite{saeedExplainableAIXAI2023, ehsan2020}.
%
% Current problems with XAI regarding user needs
However, these AI explanations are often developed by and for XAI experts, even though many end-users lack the AI knowledge of XAI experts \cite{ehsan2021, ehsan2021b}.
Recently, it has become clear that these explanations do not meet the needs of the intended users of these AI systems, but instead serve, \eg AI engineers and data scientists \cite{ehsan2021b, Liao2020}.
% ... and are ineffective in making the decisions understandable to those users .
%
% Current solution ideas
The emerging field of Human-Centered Explainable Artificial Intelligence (HC-XAI) seeks to make model decisions understandable by investigating the explanation needs of real end-users of specific domains \cite{ehsan2020}.
As per \cite{saeedExplainableAIXAI2023} there are different perspectives on the need for XAI, \eg regulatory, scientific, industrial and end-user perspectives.
Recent research suggests that understanding people's, \ie end-user's, needs is fundamental for developing XAI methods \cite{kim2023, Liao2020,liao2022humancentered, ehsan2020}. 

% Explanation Methods
%
% Different XAI needs taxonomies and Liao
Different conceptual frameworks have been developed to characterise needs for XAI, \eg based on expert opinions from different fields \cite{Mohseni2021}, stakeholders needs \cite{preece2018stakeholders, langer2021}), stakeholders knowledge and goals \cite{suresh2021a}, psychology \cite{sanneman2020, Wang2019}. Other authors used interviews to investigate user needs \cite{Hong2020, Liao2020}. 
%Wang et al. (2019), Mohseni et al. (2021) and Liao et al. (2020) based on Lim2010.
% Reasons why we use Liaos XAIQB
In this paper we focus on Liao et al. \cite{Liao2020} as they deliver a context-independent human-centered approach, which could be adapted to different scenarios. In addition, we consider this article of high interest due to its 434 citations according to google scholar (May, 2023). 
However, few studies seem to use or build on and reflect on the Liao et al.'s XAIQB directly and even less tested it empirically with user studies. This interest reinforces the need to investigate the XAIQB further.

% Description Liao's XAIQB
Liao et al. \cite{Liao2020} propose a algorithm-informed XAI question bank XAIQB) to explore real-world user needs for understanding AI. The authors conducted 20 interviews with UX and design practitioners to explore gaps in XAI algorithm work and practices. In order to do this Liao et al. used besides other conceptual works Lim and Deys \cite{Lim2010} taxonomy to support intelligibility in context-aware applications as a foundation \cite{Lim2010}. Liao et al. expanded these explainability needs categories by mapping them to explanation methods. This resulted in 9 explainability needs categories of prototypical questions users may have regarding an AI tool: Input, Output, Performance, How (global), Why, Why not, What if, How to be that, How to still be this and Others \cite{Liao2020}. 

% Studies using XAIQB
In the following section previous studies of interest using Liao et al.'s XAIQB will be shortly described.
In our literature research, we found that many papers only mention Liao et al. \cite{Liao2020} as part of a literature review \cite{antoniadi2021, chromik2021, jiménez-luna2020, kaluarachchi2021} or for theory-related arguments \cite{drozdal2020, poursabzi-sangdeh2021, shneiderman2020}. 
A few studies we identified directly used the XAIQB as a theoretical foundation.
Nguyen et al. \cite{nguyen2022a} developed a conversational agent to inform users about explanations in a manner similar to human-to-human conversations. The authors extended the XAIQB with quality-controlled paraphrases, and researched suitable XAI methods to answer these questions \cite{nguyen2022a}). Similarly, Shen et al. \cite{shen2021a} summarized common forms of explanations about natural language processing and compared them to the XAIQB \cite{shen2021a}). Liao et al. \cite{liao2021question} developed a question-driven design process including a mapping guide between user questions and XAI needs based on the XAIBQ, 21 interviews with AI practitioners and two healthcare use cases. \cite{liao2021question}).
We could only identify a few papers, which use the XAIBQ to investigate user needs empirically. Kim et al. \cite{kim2023} used the XAIQB to developed open-ended questions and a survey to research how explainability can improve human-AI interaction. 20 end-users were questioned regarding their needs about a real-world AI bird identification application. Besides the 9 categories of Liao et al. \cite{Liao2020} the question category transparency was added on a theoretical foundation \cite{kim2023}). He et al. \cite{he2023} developed a user needs library based on the XAIQB, which they adjusted to a medical context based on their literature review. Afterwards a XAI prototype in a medical context was designed and needs and preferences of consumer users regarding explanations were analyzed \cite{he2023}).
We were unable to find a study that empirically evaluates the original XAIQB directly.
%
% Erwähnte Paper von unten mit hoch nehmen







% Katrins Part Stand 05.06.2023
\section{Methods}
As part of our ongoing research into the potential of human-AI collaboration in areas such as humanities and art history, we conducted an interview study and software exploration with 12 art historians in March and April 2022.
\subsection{Study design and participants}
 In the following, we only report on the findings from the software exploration. We conducted the software exploration in order to not only capture our participants' theoretically formed preconceptions regarding computational tools, specifically regarding nonspecified AI systems but rather gain direct insights into our participants' practices of use. During the think-aloud~\cite{Lewis_1982} software exploration, the participants used a CV-based tool to conduct a real-world image retrieval task that is grounded in their current research. For this purpose, we had our participants interact with the web-based tool \texttt{imgs.ai}~\cite{imgsai2023}\footnote{Further information is provided on \url{https://imgs.ai/}.}. 
The tool allows users to perform a visual search on a selection of museum collection datasets and enables users to interactively select different embeddings, \ie compressed semantic descriptors for images, and a distance metric as a similarity criterion when performing their search ~\cite{imgsai2023}. The operation of the ready-to-use web-based search tool does not require advanced technical knowledge\footnote{We are not involved in the development of this tool but see \texttt{imgs.ai} as a typical example of a computational tool for humanities research.}. 
%
We compiled a list of potential participants that all had to hold at least one academic degree in art history and work in an art history-related profession. The initial selection of potential participants was based on our professional networks and later extended by researching art historians listed on institutional websites of universities, research institutes, museums, or other collecting institutions. We snowballed additional candidates during the first round of contacting participants. The final list included 35 potential study participants. All participants were assigned a level of familiarity with computational approaches\footnote{We assigned levels ``A - high'' to ``C - low'' based on information from their profiles on institutional or personal websites and from their publication history.} From this list, we ultimately selected 12 participants and made sure that our sample consisted of all three levels of familiarity (three participants were qualitatively grouped as `A', \ie high familiarity with computational approaches, five as `B, \ie medium familiarity with computational approaches, and four as `C,' \ie  low familiarity with computational approaches). With this sample, we aimed at reducing probable `skepticism' or `enthusiasm' bias towards computational approaches that might correlate with the level of familiarity.
%
The software exploration was conducted remotely through the video conferencing software Webex\footnote{Webex is video conference software developed by Cisco. For more information, we refer to \url{https://www.webex.com}.} which was also used to record the audio and video. Participants were informed of the circumstances of the recording and consented to it\footnote{Our university does not have an institutional or ethical review board. To compensate for this, we have developed internal guidelines that set ethical and legal standards for our research group. These guidelines include sending all potential participants a thorough information sheet upon first contacting them, which allows them to determine whether or not they are willing to participate in the study. They were also informed that they would not be compensated for participating in our study. Upon acceptance of participation and prior to the interviews, participants received another detailed information sheet that informed them about the background of the study, detailed the process and how the interview will be conducted, and how the data collected will be used and stored. The document, which is approved by our university's Chief Data Protection Officer, also informs them of their rights under the General Data Protection Regulation.}.

We had asked the participants to bring a digital image with which they could perform an image retrieval task that is relevant to their research or current work. During interaction with the tool, participants shared their screens, which allowed us to record and follow their interaction with the tool and to insert questions or provide help when needed. We only briefly introduced the tool at the beginning of the software exploration. This mimics how they would use such a tool as part of their everyday work, \ie depending on the available information and explanations integrated with the tool. The participants were instructed to verbally share their thoughts, observations, and questions that arose during the interaction, \ie to think-aloud~\cite{Lewis_1982}. We also asked them to explain their search interest and to share their interpretation of the tool's output verbally. The software explorations lasted for approximately 25 minutes and were conducted in German. 

We transcribed the audio recordings of the software exploration and consulted the video recordings of the users' screens to additionally transcribe relevant actions that were not verbalized using MAXQDA\footnote{\url{https://www.maxqda.com/}}. The software was chosen because it is widely used for qualitative data analysis and mixed methods research, and (probably most importantly) because our university provides it.
%

\subsection{Analysis procedure}
The analysis was carried out by three of the authors and consisted of three phases, preparation, coding, and refinement. In the preparation phase, we met to go through and discuss all of the XAIQB's questions. For every question we deliberated how it might be interpreted generally and for specifically our context, \eg \enquote{Beispiel}.\todo[inline]{Beispiel einfügen} Afterward, we wrote down the first draft of a definition for every question. 

We used MAXQDA again for the coding phase, where we defined all 49 XAIQB questions as codes plus an additional code \enquote{new question}. The coding took place iteratively over four rounds, with each round consisting of coding multiple software explorations (two explorations in round 1, three in rounds 2 and 3, and four in round 4) and meeting up again to discuss the assigned codes. During the inductive and deductive coding process, we made rigorous use of MAXQDA's notes feature to specify why we applied a code to a specific segment, and for the \enquote{new question} code why we think this question should be added to the XAIQB. In the discussion, we went through each code assignment and debated until we reached an agreement. The talking points of the discussion and our notes were used to refine the question definitions from the preparation phase. For each of the \enquote{new question} segments we elaborated on why this question expresses an explanation need that differs from the ones in the XAIQB. If a consensus was reached, the wording of the new question was refined, assigned a category, given a definition, and added as a code for the next rounds.

Finally, in the refinement phase, we made a plausibility check on each newly added question to evaluate if it is relevant to a general AI system and not just to our context and removed questions that did not pass this check. We also had another discussion round where we made another pass over all question definitions and refined them for clarity and general applicability.


